Delta-stepping SSSP: from Vertices and Edges to GraphBLAS Implementations

GraphBLAS is an interface for implementing graph algorithms. Algorithms implemented using the GraphBLAS interface are cast in terms of linear algebra-like operations. However, many graph algorithms are canonically described in terms of operations on vertices and/or edges. Despite the known duality between these two representations, the differences in the way algorithms are described using the two approaches can pose considerable difficulties in the adoption of the GraphBLAS as standard interface for development. This paper investigates a systematic approach for translating a graph algorithm described in the canonical vertex and edge representation into an implementation that leverages the GraphBLAS interface. We present a two-step approach to this problem. First, we express common vertex- and edge-centric design patterns using a linear algebraic language. Second, we map this intermediate representation to the GraphBLAS interface. We illustrate our approach by translating the delta-stepping single source shortest path algorithm from its canonical description to a GraphBLAS implementation, and highlight lessons learned when implementing using GraphBLAS.

==> color_flatex.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Array related wizardry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcolumntype{I}{!{\vrule width 1.5pt}}
\newlength\savedwidth
\newcommand\whline{\noalign{\global\savedwidth\arrayrulewidth
                            \global\arrayrulewidth 1.5pt}%
           \hline
           \noalign{\global\arrayrulewidth\savedwidth}}


% ----------------------------------------------------------------

% In math mode,
% \FlaTwoByTwo{A}{B}
%             {C}{D}
% creates the picture
%   / A || B \
%   | ==  == |
%   \ C || D /

\newcommand{\FlaTwoByTwo}[4]{
\left(
\begin{array}{c I c}
#1 & #2 \\ \whline
#3 & #4
\end{array}
\right)
}

\newcommand{\FlaTwoByTwoNoPar}[4]{
\begin{array}{c I c}
#1 & #2 \\ \hline
#3 & #4
\end{array}
}

\newcommand{\FlaTwoByTwoSingleLineNoPar}[4]{
\begin{array}{c | c}
#1 & #2 \\ \hline
#3 & #4
\end{array}
}

\newcommand{\FlaTwoByTwoSingleLine}[4]{
\left(
\begin{array}{c | c}
#1 & #2 \\ \hline
#3 & #4
\end{array}
\right)
}


\newcommand{\FlaTwoByTwoNoLine}[4]{
\left(
\begin{array}{c  c}
#1 & #2 \\
#3 & #4
\end{array}
\right)
}

% In math mode,
% \FlaTwoByOne{A}
%             {C}
% creates the picture
%   / A  \
%   | == |
%   \ C  /

\newcommand{\FlaTwoByOne}[2]{
\left(
\begin{array}{c}
#1 \\ \hline
#2
\end{array}
\right)
}

\newcommand{\FlaTwoByOneNoPar}[2]{
\begin{array}{c}
#1 \\ \hline
#2
\end{array}
}

% In math mode,
% \FlaTwoByOneSingleLine{A}
%                       {C}
% creates the picture
%   / A  \
%   | -- |
%   \ C  /

\newcommand{\FlaTwoByOneSingleLine}[2]{
\left(
\begin{array}{c}
#1 \\ \hline
#2
\end{array}
\right)
}

\newcommand{\FlaTwoByOneSingleLineNoPar}[2]{
\begin{array}{c}
#1 \\ \hline
#2
\end{array}
}


\newcommand{\FlaTwoByOneNoLine}[2]{
\left(
\begin{array}{c}
#1 \\
#2
\end{array}
\right)
}

% In math mode,
% \FlaOneByTwo{A}{B}
% creates the picture
%   ( A || B )

\newcommand{\FlaOneByTwo}[2]{
\left(
\begin{array}{c I c}
#1 & #2
\end{array}
\right)
}

\newcommand{\FlaOneByTwoNoPar}[2]{
\begin{array}{c I c}
#1 & #2
\end{array}
}

\newcommand{\FlaOneByTwoSingleLine}[2]{
\left(
\begin{array}{c | c}
#1 & #2
\end{array}
\right)
}

\newcommand{\FlaOneByTwoNoLine}[2]{
\left(
\begin{array}{c c}
#1 & #2
\end{array}
\right)
}

% In math mode,
% \FlaThreeByThreeTL{A}{B}{C}
%                   {D}{E}{F}
%                   {G}{H}{I}
% creates the picture
%   / A | B || C \
%   | -- ---  -- |
%   | D | E || F |
%   | ==  ==  == |
%   \ G | H || I /
% Notice: the TL means that the
% center block (E) is part of the
% TL quadrant, where quadrants are
% partitioned by the double lines.

\newcommand{\FlaThreeByThreeTL}[9]{
\left(
\begin{array}{c | c I c}
#1 & #2 & #3 \\ \hline
#4 & #5 & #6 \\ \whline
#7 & #8 & #9
\end{array}
\right)
}

\newcommand{\FlaThreeByThreeTLNoPar}[9]{
\begin{array}{c | c I c}
#1 & #2 & #3 \\ 
#4 & #5 & #6 \\ \hline 
#7 & #8 & #9 
\end{array}
}

% In math mode,
% \FlaThreeByThreeBR{A}{B}{C}
%                   {D}{E}{F}
%                   {G}{H}{I}
% creates the picture
%   / A || B | C \
%   | ==  ==  == |
%   | D || E | F |
%   | -- ---  -- |
%   \ G || H | I /
% Notice: the BR means that the
% center block (E) is part of the
% BR quadrant, where quadrants are
% partitioned by the double lines.

\newcommand{\FlaThreeByThreeBR}[9]{
\left(
\begin{array}{c I c | c}
#1 & #2 & #3 \\ \whline 
#4 & #5 & #6 \\ \hline
#7 & #8 & #9 
\end{array}
\right) 
}

\newcommand{\FlaThreeByThreeSingleLine}[9]{
\left(
\begin{array}{c | c | c}
#1 & #2 & #3 \\ \hline
#4 & #5 & #6 \\ \hline
#7 & #8 & #9
\end{array}
\right)
}

\newcommand{\FlaThreeByThreeNoLine}[9]{
\left(
\begin{array}{c c c}
#1 & #2 & #3 \\
#4 & #5 & #6 \\
#7 & #8 & #9
\end{array}
\right)
}

\newcommand{\FlaThreeByThreeBRNoPar}[9]{
\begin{array}{c I c | c}
#1 & #2 & #3 \\ \hline 
#4 & #5 & #6 \\ 
#7 & #8 & #9 
\end{array}
}

% In math mode,
% \FlaThreeByThreeTR{A}{B}{C}
%                   {D}{E}{F}
%                   {G}{H}{I}
% creates the picture
%   / A || B | C \
%   | -- ---  -- |
%   | D || E | F |
%   | ==  ==  == |
%   \ G || H | I /
% Notice: the TR means that the
% center block (E) is part of the
% TR quadrant, where quadrants are
% partitioned by the double lines.

\newcommand{\FlaThreeByThreeTR}[9]{
\left(
\begin{array}{c I c | c}
#1 & #2 & #3 \\ \hline
#4 & #5 & #6 \\ \whline
#7 & #8 & #9
\end{array}
\right)
}


% In math mode,
% \FlaThreeByThreeBL{A}{B}{C}
%                   {D}{E}{F}
%                   {G}{H}{I}
% creates the picture
%   / A | B || C \
%   | ==  ==  == |
%   | D | E || F |
%   | -- ---  -- |
%   \ G | H || I /
% Notice: the BL means that the
% center block (E) is part of the
% BL quadrant, where quadrants are
% partitioned by the double lines.

\newcommand{\FlaThreeByThreeBL}[9]{
\left(
\begin{array}{c | c I c}
#1 & #2 & #3 \\ \hline
#4 & #5 & #6 \\ 
#7 & #8 & #9
\end{array}
\right)
}

% In math mode,
% \FlaOneByThreeR{A}{B}{C}
% creates the picture
%   ( A || B | C )
% Notice: the R means that the
% center block (B) is part of the
% R(ight) submatrix, where
% submatrices are % partitioned
% by the double lines.

\newcommand{\FlaOneByThreeR}[3]{
\left(
\begin{array}{c I c | c}
#1 & #2 & #3
\end{array}
\right)
}

% In math mode,
% \FlaOneByThreeL{A}{B}{C}
% creates the picture
%   ( A | B || C )
% Notice: the R means that the
% center block (B) is part of the
% R(ight) submatrix, where
% submatrices are % partitioned
% by the double lines.

\newcommand{\FlaOneByThreeL}[3]{
\left(
\begin{array}{c | c I c}
#1 & #2 & #3
\end{array}
\right)
}

% In math mode,
% \FlaThreeByOneT{A}
%                {D}
%                {G}
% creates the picture
%   / A  \
%   | == |
%   | B  |
%   | -- |
%   \ C  /
% Notice: the T means that the
% center block (C) is part of the
% T(op) submatrix where submatrices
% are % partitioned by the double
% lines.

\newcommand{\FlaThreeByOneT}[3]{
\left(
\begin{array}{c}
#1 \\ 
#2 \\ \hline
#3
\end{array}
\right)
}

\newcommand{\FlaThreeByOneTNoPar}[3]{
\begin{array}{c}
#1 \\ 
#2 \\ \hline
#3
\end{array}
}

% In math mode,
% \FlaThreeByOneB{A}
%                {D}
%                {G}
% creates the picture
%   / A  \
%   | -- |
%   | B  |
%   | == |
%   \ C  /
% Notice: the B means that the
% center block (C) is part of the
% T(op) submatrix where submatrices
% are % partitioned by the double
% lines.

\newcommand{\FlaThreeByOneB}[3]{
\left(
\begin{array}{c}
#1 \\ \hline
#2 \\ 
#3
\end{array}
\right)
}

\newcommand{\FlaThreeByOneBNoPar}[3]{
\begin{array}{c}
#1 \\ \hline
#2 \\ 
#3
\end{array}
}

\newcommand{\FlaThreeByOneSingleLine}[3]{
\left(
\begin{array}{c}
#1 \\ \hline
#2 \\ \hline
#3
\end{array}
\right)
}

\newcommand{\FlaThreeByOneNoLine}[3]{
\left(
\begin{array}{c}
#1 \\
#2 \\
#3
\end{array}
\right)
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\operation}{}

\newcommand{\routinename}{}

\newcommand{\precondition}{~}

\newcommand{\postcondition}{~}

\newcommand{\invariant}{~}

\newcommand{\guard}{~}

\newcommand{\partitionings}{~}

\newcommand{\partitionsizes}{~}

\newcommand{\blocksize}{blank}

\newcommand{\repartitionings}{~}

\newcommand{\repartitionsizes}{~}

\newcommand{\moveboundaries}{~}

\newcommand{\beforeupdate}{~}

\newcommand{\afterupdate}{~}

\newcommand{\update}{~}

%%%%%%%%%%%%%%

\newcommand{\resetsteps}{

\renewcommand{\operation}{\phantom{[A] = op( A )}}

\renewcommand{\routinename}{\operation}

\renewcommand{\precondition}{\phantom{A = \widehat A}}

\renewcommand{\postcondition}{\phantom{A = \widehat A}}

\renewcommand{\invariant}{\phantom{ 
	  \left(\begin{array}{c}
	y_T \\ \whline
	y_B 
	\end{array}\right) 
	\rightarrow
	\left(\begin{array}{c}
	y_0 \\ \whline 
	\psi_1 \\  
	y_2
	\end{array}\right) \hspace{3in}\mbox{~}
		}
}

\renewcommand{\blocksize}{blank}

\renewcommand{\guard}{\phantom{m( A_{BL} ) < m( A )}}

\renewcommand{\partitionings}{
$
\phantom{\FlaTwoByTwo{A_{TL}}{A_{TR}}{A_{BL}}{A_{BR}}
\rightarrow
\FlaThreeByThreeBR
   {A_{00}}{a_{01}}{A_{02}}
   {a_{10}^T}{\alpha_{11}}{a_{12}^T}
   {A_{20}}{a_{21}}{A_{22}}}   
$
}

\renewcommand{\partitionsizes}{$ \phantom{m( A )} $}

\renewcommand{\repartitionings}{
$
\phantom{\FlaTwoByTwo{A_{TL}}{A_{TR}}{A_{BL}}{A_{BR}}
\rightarrow
\FlaThreeByThreeBR
   {A_{00}}{a_{01}}{A_{02}}
   {a_{10}^T}{\alpha_{11}}{a_{12}^T}
   {A_{20}}{a_{21}}{A_{22}}}   
$
}

\renewcommand{\repartitionsizes}{$\phantom{m(A)}$}

\renewcommand{\moveboundaries}{
$
\phantom{\FlaTwoByTwo{A_{TL}}{A_{TR}}{A_{BL}}{A_{BR}}
\rightarrow
\FlaThreeByThreeBR
   {A_{00}}{a_{01}}{A_{02}}
   {a_{10}^T}{\alpha_{11}}{a_{12}^T}
   {A_{20}}{a_{21}}{A_{22}}}   
$
}

\renewcommand{\beforeupdate}{
\phantom{$\FlaTwoByTwo{A_{TL}}{A_{TR}}{A_{BL}}{A_{BR}}
\rightarrow
\FlaThreeByThreeBR
   {A_{00}}{a_{01}}{A_{02}}
   {a_{10}^T}{\alpha_{11}}{a_{12}^T}
   {A_{20}}{a_{21}}{A_{22}}$}   
}

\renewcommand{\afterupdate}{
\phantom{$\FlaTwoByTwo{A_{TL}}{A_{TR}}{A_{BL}}{A_{BR}}
\rightarrow
\FlaThreeByThreeBR
   {A_{00}}{a_{01}}{A_{02}}
   {a_{10}^T}{\alpha_{11}}{a_{12}^T}
   {A_{20}}{a_{21}}{A_{22}}$}   
}

\renewcommand{\update}{
\phantom{$
\begin{array}{l}
\\
\\
\\
\end{array}
$}
}
}

\newcommand{\NoShow}[1]{}



\newcommand{\FlaAlgorithm}{
\begin{tabular}{|l|} \hline
$\mbox{\color{blue}Algorithm:~}\routinename$
\\ \whline
\partitionings \\
$\mbox{\color{blue} ~~~where~}$ \partitionsizes 
\\ 
$\mbox{\color{blue}while~} \ShowGuard \mbox{~\color{blue} do}$
\\
\ifthenelse{\equal{\blocksize}{1}}{}%
{%
\ifthenelse{ \equal{\blocksize}{blank} }{}%
{~~~~{\bf Determine block size $ \blocksize $}\\}%
}
~~~~ 
\repartitionings \\
~~~$\mbox{\color{blue} ~~~where~}$ \repartitionsizes
\\ \hline
~~~~  \update 
\\ \hline
~~~~ 
\moveboundaries 
\\
$\mbox{\color{blue} endwhile} $
\\ \hline 
\end{tabular}
}


\newcounter{WSStep}
\setcounter{WSStep}{9}

\newcommand{\ShowPrecondition}{\ifthenelse{\value{WSStep}<1}%
   {{\color{white} \precondition}}
   {\ifthenelse{\value{WSStep}=1}%
    {\color{red} \precondition}
    {\color{black} \precondition}}}
\newcommand{\ShowPostcondition}{\ifthenelse{\value{WSStep}<1}%
   {{\color{white} \postcondition}}
   {\ifthenelse{\value{WSStep}=1}%
    {\color{red} \postcondition}
    {\color{black} \postcondition}}}
\newcommand{\ShowInvariant}{\ifthenelse{\value{WSStep}<2}%
   {{\color{white} \invariant}}
   {\ifthenelse{\value{WSStep}=2}%
    {\color{red} \invariant}
    {\color{black} \invariant}}}
\newcommand{\ShowGuard}{\ifthenelse{\value{WSStep}<3}%
   {{\color{lightgray!25} \guard}}
   {\ifthenelse{\value{WSStep}=3}%
    {\color{red} \guard}
    {\color{black} \guard}}}
\newcommand{\ShowGuardTwo}{\ifthenelse{\value{WSStep}<3}%
   {{\color{white} \guard}}
   {\ifthenelse{\value{WSStep}=3}%
    {\color{red} \guard}
    {\color{black} \guard}}}
\newcommand{\ShowPartitionings}{\ifthenelse{\value{WSStep}<4}%
   {{\color{lightgray!25} \partitionings}}%
   {\ifthenelse{\value{WSStep}=4}%
    {\color{red} \partitionings}%
    {\color{black} \partitionings}}}
\newcommand{\ShowPartitionSizes}{\ifthenelse{\value{WSStep}<4}%
   {{\color{lightgray!25} \partitionsizes}}
   {\ifthenelse{\value{WSStep}=4}%
    {\color{red} \partitionsizes}
    {\color{black} \partitionsizes}}}
\newcommand{\ShowRepartitionings}{\ifthenelse{\value{WSStep}<5}%
   {{\color{lightgray!25} \repartitionings}}
   {\ifthenelse{\value{WSStep}=5}%
    {\color{red} \repartitionings}
    {\color{black} \repartitionings}}}
\newcommand{\ShowRepartitionSizes}{\ifthenelse{\value{WSStep}<5}%
   {{\color{lightgray!25} \repartitionsizes}}
   {\ifthenelse{\value{WSStep}=5}%
    {\color{red} \repartitionsizes}
    {\color{black} \repartitionsizes}}}
\newcommand{\ShowMoveBoundaries}{\ifthenelse{\value{WSStep}<5}%
   {{\color{lightgray!25} \moveboundaries}}
   {\ifthenelse{\value{WSStep}=5}%
    {\color{red} \moveboundaries}
    {\color{black} \moveboundaries}}}
\newcommand{\ShowBeforeUpdate}{\ifthenelse{\value{WSStep}<6}%
   {{\color{white} \beforeupdate}}
   {\ifthenelse{\value{WSStep}=6}%
    {\color{red} \beforeupdate}
    {\color{black} \beforeupdate}}}
\newcommand{\ShowAfterUpdate}{\ifthenelse{\value{WSStep}<7}%
   {{\color{white} \afterupdate}}
   {\ifthenelse{\value{WSStep}=7}%
    {\color{red} \afterupdate}
    {\color{black} \afterupdate}}}
\newcommand{\ShowUpdate}{\ifthenelse{\value{WSStep}<8}%
   {{\color{lightgray!25} \update}}
   {\ifthenelse{\value{WSStep}=8}%
    {\color{red} \update}
    {\color{black} \update}}}
   



\newcommand{\FlaWorksheet}{
\begin{tabular}{| c | p{0.9\textwidth} |}\hline
Step & $\mbox{\color{blue}Algorithm:~}\routinename$
\\ \hline
1a &%
$ \left\{ 
\begin{minipage}{0.88\textwidth} 
$\ShowPrecondition$  
\end{minipage}
\right\}
$%
\\ \hline
\rowcolor{lightgray!25}   
4 & %
\begin{minipage}{0.88\textwidth}%
\vspace{0.05in}
\ShowPartitionings~ \\
\mbox{\color{blue} ~~~where~} \ShowPartitionSizes
\end{minipage}
\\ \hline
2 & 
$ \left\{ 
\begin{minipage}{0.88\textwidth} 
$\ShowInvariant $
\end{minipage}
\right\} $ 
\\ \hline
\rowcolor{lightgray!25}   
3 &$\mbox{\color{blue}while~} \ShowGuard \mbox{~\color{blue} do}$
\\ \hline 
2,3 &  
$
\left\{
\begin{minipage}[t]{0.88\textwidth}%
~~~~$
\ShowInvariant  
\wedge \ShowGuardTwo
$
\end{minipage}
\right\}
$ 
\\ \hline
\rowcolor{lightgray!25}   
5a & ~~~~ \begin{minipage}{0.85\textwidth}%
\vspace{0.05in}
\ifthenelse{\equal{\blocksize}{1}}{}%
{%
\ifthenelse{ \equal{\blocksize}{blank} }{}%
{{\bf Determine block size $ \blocksize $}\\}%
}
\ShowRepartitionings~ \\
$\mbox{\color{blue} ~~~where~}$ \ShowRepartitionSizes
\end{minipage}
\\ \hline
6 & 
$ \left\{ 
\begin{minipage}{0.88\textwidth} 
~~~~ \ShowBeforeUpdate 
\end{minipage}
\right\}
$
\\ \hline
\rowcolor{lightgray!25}  
8 & ~~~~  \ShowUpdate 
\\ \hline 
7 & 
$ \left\{ 
\begin{minipage}{0.88\textwidth} 
 ~~~~ \ShowAfterUpdate 
\end{minipage}
\right\}
$
\\ \hline
\rowcolor{lightgray!25}   
5b & ~~~~ \begin{minipage}{0.85\textwidth}%
\vspace{0.05in}
\ShowMoveBoundaries~
\end{minipage}
\\ \hline
2 & 
$ \left\{ 
\begin{minipage}{0.88\textwidth} 
~~~~ $ \ShowInvariant  $ 
\end{minipage}
\right\}
$
\\ \hline
\rowcolor{lightgray!25}  
 &$\mbox{\color{blue} endwhile} $
\\ \hline 
2,3 & 
$ \left\{ 
\begin{minipage}{0.88\textwidth} 
$ 
\ShowInvariant 
\wedge \neg( \ShowGuardTwo )
$
\end{minipage}
\right\}
$
\\ \hline
1b & 
$ \left\{ 
\begin{minipage}{0.88\textwidth} 
$ \ShowPostcondition $ 
\end{minipage}
\right\}
$
\\ \hline
\end{tabular}
}



\newcommand{\FlaWorksheetNine}{
\begin{tabular}{| c | p{0.9\textwidth} |}\hline
{\color{white}Step} & $\mbox{\color{blue}Algorithm:~}\routinename$
\\ \hline
 &%
$ \phantom{\left\{ 
\begin{minipage}{0.88\textwidth} 
$\ShowPrecondition$  
\end{minipage}
\right\}}
$%
\\ \hline
\rowcolor{lightgray!25}   
& %
\begin{minipage}{0.88\textwidth}%
\vspace{0.05in}
\ShowPartitionings~ \\
\mbox{\color{blue} ~~~where~} \ShowPartitionSizes
\end{minipage}
\\ \hline
& 
$ \phantom{\left\{ 
\begin{minipage}{0.88\textwidth} 
$\ShowInvariant $
\end{minipage}
\right\}} $ 
\\ \hline
\rowcolor{lightgray!25}   
&$\mbox{\color{blue}while~} \ShowGuard \mbox{~\color{blue} do}$
\\ \hline 
 &  
$
\phantom{\left\{
\begin{minipage}[t]{0.88\textwidth}%
~~~~$
\ShowInvariant 
\wedge \ShowGuardTwo$
\end{minipage}
\right\}}
$ 
\\ \hline
\rowcolor{lightgray!25}   
 & ~~~~ \begin{minipage}{0.85\textwidth}%
\vspace{0.05in}
\ifthenelse{\equal{\blocksize}{1}}{}%
{%
\ifthenelse{ \equal{\blocksize}{blank} }{}%
{{\bf Determine block size $ \blocksize $}\\}%
}
\ShowRepartitionings~ \\
$\mbox{\color{blue} ~~~where~}$ \ShowRepartitionSizes
\end{minipage}
\\ \hline
& 
$ \phantom{\left\{ 
\begin{minipage}{0.88\textwidth} 
~~~~ \ShowBeforeUpdate 
\end{minipage}
\right\}}
$
\\ \hline
\rowcolor{lightgray!25}  
 & ~~~~  \ShowUpdate 
\\ \hline 
& 
$ \phantom{\left\{ 
\begin{minipage}{0.88\textwidth} 
~~~~ \ShowAfterUpdate 
\end{minipage}
\right\}}
$
\\ \hline
\rowcolor{lightgray!25}   
 & ~~~~ \begin{minipage}{0.85\textwidth}%
\vspace{0.05in}
\ShowMoveBoundaries~
\end{minipage}
\\ \hline
& 
$ \phantom{\left\{ 
\begin{minipage}{0.88\textwidth} 
~~~~ $ \ShowInvariant  $ 
\end{minipage}
\right\}}
$
\\ \hline
\rowcolor{lightgray!25}  
 &$\mbox{\color{blue} endwhile} $
\\ \hline 
& 
$ \phantom{\left\{ 
\begin{minipage}{0.88\textwidth} 
$ \ShowInvariant \wedge \neg( \ShowGuardTwo )$ 
\end{minipage}
\right\}}
$
\\ \hline
& 
$ \phantom{\left\{ 
\begin{minipage}{0.88\textwidth} 
$ \ShowPostcondition $ 
\end{minipage}
\right\}}
$
\\ \hline
\end{tabular}
}


\newcommand{\FlaWorksheetEight}{
\setcounter{WSStep}{8}
\FlaWorksheet 
\setcounter{WSStep}{9}
}


\newcommand{\FlaWorksheetSeven}{
\setcounter{WSStep}{7}
\FlaWorksheet 
\setcounter{WSStep}{9}
}


\newcommand{\FlaWorksheetSix}{
\setcounter{WSStep}{6}
\FlaWorksheet 
\setcounter{WSStep}{9}
}


\newcommand{\FlaWorksheetFive}{
\setcounter{WSStep}{5}
\FlaWorksheet 
\setcounter{WSStep}{9}
}


\newcommand{\FlaWorksheetFour}{
\setcounter{WSStep}{4}
\FlaWorksheet 
\setcounter{WSStep}{9}
}


\newcommand{\FlaWorksheetThree}{
\setcounter{WSStep}{3}
\FlaWorksheet 
\setcounter{WSStep}{9}
}


\newcommand{\FlaWorksheetTwo}{
\setcounter{WSStep}{2}
\FlaWorksheet 
\setcounter{WSStep}{9}
}


\newcommand{\FlaWorksheetOne}{
\setcounter{WSStep}{1}
\FlaWorksheet 
\setcounter{WSStep}{9}
}


\newcommand{\FlaWorksheetZero}{
\setcounter{WSStep}{0}
\FlaWorksheet 
\setcounter{WSStep}{9}
}


\newcommand{\PseudocodeAssert}[1]{%
%
$%
\left\{ 
\colorbox{white}{
	\begin{minipage}{0.9\textwidth}
#1 
\end{minipage}%
}
\right\}  
$
\\ \hline 
}

\newcommand{\PseudocodeAssertColor}[2]{%
%
$%
\left\{ 
\colorbox{#1}{
	\begin{minipage}{0.9\textwidth}
#2
\end{minipage}%
}
\right\}  
$
\\ \hline 
}

\newcommand{\PseudocodeAssertBlank}[1]{%
%
%
$%
\left\{ 
\colorbox{white}{
	\phantom{\raisebox{0pt}[2em][2em]{\begin{minipage}{0.9\textwidth}
#1 
\end{minipage}}}
}
\right\}  
$
\\ \hline 
}

\newcommand{\PseudocodeAssertNotBlank}[1]{%
%
%
$%
\left\{ 
\colorbox{white}{
	{\raisebox{0pt}[2em][2em]{\begin{minipage}{0.9\textwidth}
#1 
\end{minipage}}}
}
\right\}  
$
\\ \hline 
}

\newcommand{\PseudocodeAssertIndent}[1]{%
\cellcolor{white}%
\mbox{~~~~} % 
$%
\left\{ 
\cellcolor{white}{
	\begin{minipage}{0.9\textwidth}
#1
\end{minipage}
}
\right\}  
$
\\ \hline 
}

\newcommand{\PseudocodeAssertIndentColor}[2]{%
\cellcolor{#1}%
\mbox{~~~~} % 
$%
\left\{ 
\cellcolor{#1}{
	\begin{minipage}{0.9\textwidth}
#2
\end{minipage}
}
\right\}  
$
\\ \hline 
}


\newcommand{\PseudocodeAssertIndentBlank}[1]{%
\cellcolor{white}%
\mbox{~~~~} % 
$%
\left\{ 
\phantom{
	\begin{minipage}{0.9\textwidth}
\raisebox{0pt}[2em][2em]{%
#1 
}
\end{minipage}}
\right\}  
$
\\ \hline 
}

\newcommand{\PseudocodeAssertIndentNotBlank}[1]{%
\cellcolor{white}%
\mbox{~~~~} % 
$%
\left\{ 
{
	\begin{minipage}{0.9\textwidth}
\raisebox{0pt}[2em][2em]{%
#1 
}
\end{minipage}}
\right\}  
$
\\ \hline 
}

\newcommand{\PseudocodeStatementColor}[2]{
	\rowcolor{lightgray!25}
%
        \begin{tabular}{@{}l}
	\colorbox{#1}{#2}
        \end{tabular}
	\\ \hline
}


\newcommand{\PseudocodeStatement}[1]{
	\rowcolor{lightgray!25}
%
        \begin{tabular}{@{}l}
	#1
        \end{tabular}
	\\ \hline
}


\newcommand{\PseudocodeStatementBlank}[1]{
	\rowcolor{lightgray!25}
\raisebox{0pt}[2em][2em]{%
        \begin{tabular}{@{}l}
	\phantom{#1}
        \end{tabular}
}
	\\ \hline 
}

\newcommand{\PseudocodeStatementNotBlank}[1]{
	\rowcolor{lightgray!25}
\raisebox{0pt}[2em][2em]{%
        \begin{tabular}{@{}l}
	{#1}
        \end{tabular}
}
	\\ \hline 
}

\newcommand{\PseudocodeStatementIndentColor}[2]{
	\rowcolor{lightgray!25}
\mbox{~~~~}
        \begin{tabular}{@{}l}
	\colorbox{#1}{#2}
        \end{tabular}
	\\ \hline
}

\newcommand{\PseudocodeStatementIndent}[1]{
	\rowcolor{lightgray!25}
\mbox{~~~~}
        \begin{tabular}{@{}l}
	#1
        \end{tabular}
	\\ \hline
}
\newcommand{\PseudocodeStatementIndentBlank}[1]{
	\rowcolor{lightgray!25}
\mbox{~~~~}
\raisebox{0pt}[2em][2em]{%
        \begin{tabular}{@{}l}
	\phantom{#1}
        \end{tabular}
}
	\\ \hline 
}


\newcommand{\PseudocodeStatementIndentNotBlank}[1]{
	\rowcolor{lightgray!25}
\mbox{~~~~}
\raisebox{0pt}[2em][2em]{%
        \begin{tabular}{@{}l}
	{#1}
        \end{tabular}
}
	\\ \hline 
}


\newenvironment{Pseudocode}{
      \begin{center}
      \begin{tabular}{ | p{0.95\textwidth} | } \hline
}
{
      \end{tabular}
      \end{center}
}
